ResUNet++: An Advanced Architecture for Medical Image Segmentation

Accurate computer-aided polyp detection and segmentation during colonoscopy examinations can help endoscopists resect abnormal tissue and thereby decrease chances of polyps growing into cancer. Towards developing a fully automated model for pixel-wise polyp segmentation, we propose ResUNet++, which is an improved ResUNet architecture for colonoscopic image segmentation. Our experimental evaluations show that the suggested architecture produces good segmentation results on publicly available datasets. Furthermore, ResUNet++ significantly outperforms U-Net and ResUNet, two key state-of-the-art deep learning architectures, by achieving high evaluation scores with a dice coefficient of 81.33%, and a mean Intersection over Union (mIoU) of 79.27% for the Kvasir-SEG dataset and a dice coefficient of 79.55%, and a mIoU of 79.62% with CVC-612 dataset.

==> augmentation.tex <==
% %%%%%%%%%%%%%%%%%%%%%image augmentation%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{figure}
%     \centering
%     \includegraphics[width=2cm, height=2cm]{figures/augmentation/1.jpg}
%     \includegraphics[width=2cm, height=2cm]{figures/augmentation/2.jpg}
%     \includegraphics[width=2cm, height=2cm]{figures/augmentation/3.jpg}
%     \includegraphics[width=2cm, height=2cm]{figures/augmentation/4.jpg} \\
%     \vspace{1mm}
%     \includegraphics[width=2cm, height=2cm]{figures/augmentation/5.jpg}
%     \includegraphics[width=2cm, height=2cm]{figures/augmentation/6.jpg}
%     \includegraphics[width=2cm, height=2cm]{figures/augmentation/7.jpg}
%     \includegraphics[width=2cm, height=2cm]{figures/augmentation/8.jpg}\\
%     \caption{A sample of the augmented images from the Kvasir-SEG dataset. From left: original, center crop, random crop, horizontal flip, vertical flip, scale augmentation, random rotation, and cutout.}
%     \label{fig:augmentation}
% \end{figure}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> cross-data.tex <==
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%cross-dataset evaluation results %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{figure}
%     \centering
%     \includegraphics [width=8cm, height=2cm]{resunet++_worstmap.jpeg}
%      %\includegraphics [width=4cm, height=4cm]{resunet++_mask1.jpg}
%     \caption{Failure case on the \resunetplusplus on the same Kvasir-SEG dataset. \textbf{(Draft: will be replaced by 2 figures)}}
%   \label{irregular_polyp}
% \end{figure}

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \begin{figure}
%     \centering
%     \includegraphics [width=8cm, height=2cm]{resunet++_worstmap.jpeg}
%     \caption{Failure case on the \resunetplusplus during cross-data evaluation. \textbf{(Draft: will be replaced by 2 figures)}}
%   \label{fig:worst_case}
% \end{figure}

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> cross-data_results_comparison.tex <==
% \begin{figure*}
%     \centering
%     \includegraphics [width=16cm, height=2cm]{cd/mask_46.jpg}\vspace{1mm}\\
%     \includegraphics [width=16cm, height=2cm]{cd/mask_48.jpg}\vspace{1mm}\\
%     \includegraphics [width=16cm, height=2cm]{cd/mask_53.jpg}\vspace{1mm}\\
%     \includegraphics [width=16cm, height=2cm]{cd/mask_55.jpg}\vspace{1mm}\\
%     \includegraphics [width=16cm, height=2cm]{cd/mask_58.jpg}\\
%     \caption{Qualitative analysis of the cross-dataset results (The model is trained on the CVC-612 and tested on Kvasir-SEG dataset). From the left: image (1), (2) ground truth, (3) U-Net, (4) ResUNet, (5) ResUNet-mod, and (6) \resunetplusplus. The proposed \resunetplusplus model produces better segmentation map than any other compared architecture.} 
%   \label{fig:comparison_with_cross_dataset}
% \end{figure*}


==> figures/T1contour.tex <==
\begin{figure}[t]
    \includegraphics[width=\linewidth]{images/MCROI_bw_screen.png}
    \caption{Example of left ventricular contours delineated on a 2D short axis T1 mapping MRI image (main panel on the right) as well as additional statistics about pixel intensity distribution (left panels).}
    \label{fig:T1contour}
\end{figure}

==> figures/T1train.tex <==
\begin{figure}
    \centering
    \begin{subfigure}[b]{0.23\textwidth}
        \includegraphics[width=\textwidth]{images/Repeats_vs_consensus_HP_t1.png}
        \caption{}
        \label{fig:T1rep}
    \end{subfigure},
     \begin{subfigure}[b]{0.22\textwidth}
        \includegraphics[width=\textwidth]{images/ColourCoded_Impact_SCMR.png}
        \caption{}
        \label{fig:T1impact}
    \end{subfigure}
    \caption{(a) Average discrepancy from consensus T1 values ($ms$) over multiple repeats of analysis for an operator. (b) Before and after training impact plot of the whole team of operators. }\label{fig:T1train}
\end{figure}

==> figures/mri_example.tex <==
%\begin{figure}[t!]
%  \includegraphics[width=\linewidth, height=\linewidth]{images/example.png}
%  \caption{Example MRI taken from the dataset supplied by Oxfords OCMR Corelab. Note that hte presented image has been resized for the purpose of this figure.}
%  \label{fig:mri_example}
%\end{figure}

==> figures/t2c.tex <==
\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{images/trainee_to_expert.png}
    \caption{Overview of the architecture for the trainee to consent method.}
    \label{fig:t2c}
\end{figure}

==> figures/training_process.tex <==
%\begin{figure*}[t]
%    \centering
 %   \includesvg[width=\textwidth]{images/ACM_Diagram}
    % \includegraphics[width=\linewidth]{images/trainee_to_consent.png}
 %   \caption{A diagram showing the entire process for training the "expert" consensus \gls{cnn} used to evaluated trainees. Starting from the left, we see that the input image is resized to $224\times224\times3$ before being put into the model. Then, the model outputs a vector with size $52,024$, which is then reshaped into the same shape as the input image. Lastly, some post-processing is applied to smooth out the segmentation and produce the contours. \textcolor{red}{NOTE!!! FIGURE MUST BE CHANGED !!!}}
%    \label{fig:training_process}
%\end{figure*}

% \begin{figure}[h]
%     \centering
%     \includegraphics[width=\linewidth]{images/trainee_to_consent.png}
%     \caption{Overview of the architecture for the trainee to expert method.}
%     \label{fig:t2e}
% \end{figure}

==> images/Polyps_type.tex <==
% \begin{figure}
%     \centering
%     \includegraphics[width=2cm, height=2cm]{images/1.jpg}
%     \includegraphics[width=2cm, height=2cm]{images/2.jpg}
%     \includegraphics[width=2cm, height=2cm]{images/3.jpg}
%     \includegraphics[width=2cm, height=2cm]{images/4.jpg}\\
%     \vspace{1mm}
%     \includegraphics[width=2cm, height=2cm]{images/5.jpg}
%     \includegraphics[width=2cm, height=2cm]{images/6.jpg}
%     \includegraphics[width=2cm, height=2cm]{images/7.jpg}
%     \includegraphics[width=2cm, height=2cm]{images/8.jpg}
%     \caption{Example images showing the variations in shape, size, color, and appearance of polyps from Kvasir-SEG dataset. Some of the images may also have bleeding and abnormal pattern over the surface of the polyp.}
%     \label{fig:polyp_shapes}
% \end{figure}



==> reviwers_comment.tex <==

%%%%%%%%%%%%%%%%%%%%----------------------- REVIEW 1 %%%%%%%%%%%%%%%%%%%%

- The title of your paper is very general. Contrary to this, your content explores a very specific segmentation problem and application area. This should be clarified - I'd recommend a title change to achieve this.

we have to fix this together. 

- The narrative could be improved in places. Your research novelty, and justification, could be better presented in the introductory section.  How and why specifically do you expand upon the existing architecture, and what are the (theoretically grounded) reasons for doing this?  The related literature section could be more critical and evaluative in nature. This would allow stronger conclusions to be carried forward to justify your methodology.



- Not all acronyms are introduced and explained.


- Fig 3 is difficult to interpret. There are two different shades of blue in the diagram (BN and Pooling).  Clarify whether these are both novel contributions on your part or if it's only ASPP.

----Solved
----------------------- REVIEW 2 ---------------------
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
The evaluation of polyp segmentation in images from colonoscopy clearly is an interesting and relevant problem in the multimedia domain. The proposed ResUNet++ architecture is interesting and the evaluation with several different datasets is sound and promising. However, the paper also raises a few questions to a reader:

1) How was the data augmentation performed in detail? For example, what values were used as rotation angles - any random integer (or float?) value between 0..359?; or just values from predefined steps? Same questions for scaling and cropping - how exactly was it performed? Also, was there any check whether the data augmentation methods were label-preserving or not?

The rotation angle is randomly chosen between 0 to 90 degree. 


2) Was there any threshold for considering IoU - e.g., such as 50\%, which is often used in the literature of object segmentation? Is this the t threshold that is mentioned in Equation 2 (which is not sufficiently described)? How exactly was the mean IoU computed? BTW: is IoU in Table III and IV also the "mean IoU"?
---------------Resolved-----------------------------------


3) Why is the performance at cross-dataset evaluation so much worse when training with CVC-612 and testing with Kvasir-SEG? (IoU 69\% vs 46\%) Similarly, why does a Kvasir-SEG trained model perform so much worse for CVC-12K? It would be good if this is somehow discussed in the paper!

-------------Resolved----------------------------

4) I wonder why only CVC-612 has been used as a training setting when evaluating with Kvasir-SEG? Why not CVC-12K, which is obviously much larger?

-------------Resolved----------------------------
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
----------------------- REVIEW 3 ---------------------
This paper proposed a new architecture, ResUNet++, for image segmentation purpose. It's based on the ResUNet structure and added squeeze and excite units, Atrous Spatial Pyramidal Pooling (ASPP), and attention units at different places in ResUNet. The network size increased dramatically because of these added units, and therefore requires longer training time.

-------------Resolved----------------------------

The authors performed comparisons of their method with the original UNet, and ResUNet on a few polyp segmentation datasets for Colorectal Cancer detection. ResUNet showed marginal improvements over the two previously proposed methods, and also better performance for cross-data generalization, when the network is trained on one dataset and tested on a different one.  Although the cross-data generalization performance are still poorer than testing on the same dataset.

-------------Resolved----------------------------

One thing I noticed is that the ResUNet doesn't perform well in the author's results, even with some modifications. The original UNet outperforms ResUNet significantly.  I wonder if the modifications the authors made to ResUNet are applicable to UNet, which seems a better place to start.

-------------Resolved----------------------------

==> takeout.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%Introduction%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Abstract}
% HDJ: This is the same as the intro. Abstract should be more straight to the point.
%Colorectal cancer is one of the leading causes of deaths worldwide. Colonoscopy using a flexible camera is the gold screening standard, but the anomaly detection rates have large potentials for improvements. Therefore,  

%Polyp of the gastrointestinal tract is the precursor for colorectal cancer. Polyp segmentation and detection in colonoscopy images plays a vital role in early detection of colorectal cancer. 

% Our model utilizes the power of U-Net, residual unit, squeeze and excitation unit, atrous spatial pyramidal pooling, and attention unit.


%Computer assisted diagnosis (CAD) can be beneficial for the examination of the patient.

%The proposed method identified polyp images from nonpolyp images in the beginning followed by predicting the polyp histology.
%The work inspired by the success of U-Net and its variant architecture as a potential solution for biomedical task.

%The models' ability to detect polyps under different conditions is an essential criterion for having it accepted at prospective clinical trials. Therefore, the models are trained on one dataset and tested on different diverse datasets to build a more generalized model. The proposed architecture may help in improving the clinical understanding of polyp by providing comprehensive insights into the location and area covered by polyp. 

\subsection{Introduction}




%Semantic segmentation is one of the fundamental topics in computer vision. The goal of the semantic segmentation task is to assign each pixel of the image with a class label. 

%In the era of big data, high computing power, and the success of a new machine learning/deep learning algorithm medical image processing has gained remarkable popularity. Gastrointestinal tract cancer are one of the leading cause of the cancer worldwide and are significant barrier to the increasing life expectancy.


%As shown in Figure~\ref{fig:polyp_shapes}, the histology of the different polyp types can look similar while at the same time the histology within one type can also be very different. Nevertheless, there is still high potential for increasing the performance of the system to clinical acceptability. 



Colonoscopy is the preferred technique for colon cancer screening and prevention. The goal of colonoscopy is to find and remove colonic polyps—precursors to colon cancer.

Polyps, as shown in Fig. 1, can appear with substantial variations in color, shape, and size.


Image quality assessment can have a major role in objective quality assessment of colonoscopy procedures. Typically, a colonoscopy video contains a large number of non-informative images with poor colon visualization that are not suitable for
inspecting the colon or performing therapeutic actions.

https://arxiv.org/pdf/1706.00712.pdf

%Unlike other natural images task, medical image segmentation task is challenging as it requires a higher level of performance. Therefore, we must develop an effective algorithm that is accurate, fast and capable of recovering fine details of the target image. \par
%Medical image analysis has already gained attention in clinical settings because they help physician in disease diagnosis. 


% Both handcrafted and state-of-art CNNs were used in the Medical Image Computing and Computer Assisted Intervention (MICCAI)  challenge for increasing the polyp detection rate. They concluded that combining both methodologies leads to an increase in the overall performance of the system.

%%%%%%%%%%%%%%%%%%%%%%%Discussion%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Related work}

%The upsampling part of the U-Net has a large number of feature channels that helps the network to propagate contextual information to the upper layer, and hence the architecture is formed as U-shaped. 

%SENet was used at ILSVRC 2017 competition, and this network improved the results of 2016 winning entry by $\sim$25\% and reduced the top-5 error to 2.251\%. Besides these improvements, the computational cost of the network is very low, and they can be added easily to the existing model. 

Tajabakash et al.~\cite{tajbakhsh2016convolutional} used  CNN to analyze and address the question of whether a full training or a fine-tuning \ac{CNN} approach works better for medical imaging applications. Their experiment on three different datasets showed that fine-tuning pre-trained network outperforms fully trained CNN from scratch or in the worst case, performed at least \ac{CNN} trained from scratch.

Brandao et al.~\cite{brandao2018towards} proposed an automatic approach for polyp detection and segmentation by restructuring the pre-trained networks such as VGG and ResNet and converted them into FCN and fine-tune them for solving the segmentation problem.


%Tajabakash et al.~\cite{tajbakhsh2016convolutional} used  CNN to analyze and address the question of whether a full training or a fine-tuning \ac{CNN} approach works better for medical imaging applications. Their experimental results demonstrated the use of pre-trained \ac{CNN} with fine-tuning for medical applications.

It is to be noted that adenomas should be removed whereas hyperplastic can be left in situ.



 %Our proposed architecture is a combination of U-Net \cite{zhang2018road}, Residual block, squeeze and excitation block \cite{hu2018squeeze}, Atrous spatial pyramid pooling \cite{chen2018deeplab}, and attention block \cite{li2019connection}. The ResUNet++ architecture takes the advantage cascaded network and boosts the performance over U-Net and ResUNet for the polyp segmentation problem. \par

%\PH{here it would be nice to end by pointing out what is still the problem of related approaches - as a motivation for your work coming next.}


%Most systems either perform frame-wise or bounding box-based detection. This is sufficient for findings polyps but to be able to determine the exact positions and types it would be important to detect each pixel of the polyp. Therefore, we aim to develop an efficient segmentation model capable of identifying fine details of the target polyp image during disease diagnosis.

%To overcome the shortcomings of the existing semantic segmentation approaches, we propose a robust and efficient architecture for medical image segmentation. In addition, we release an open dataset, Kvsir-SEG, that consists of 1,000 polyp images and their corresponding ground-truth to foster comparable and reproducible research. We also investigate how to build better generalizable models that are able to learn the semantic of the findings and not the dataset specfic features.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Proposed Method}
Hence, our model consists of an encoder, decoder, and a bridge connecting them. To improve the performance of the ResU-Net 

We replace the plain neural unit used in the U-Net with residual unit along with identity mapping. The residual blocks propagate information over layers, allowing us to build deeper networks and solving the problem of degradation that could have been caused while going deeper by the plain neural network used in U-Net.

%In total we have 15 convolutional layers comparing with 23 layers of U-Net. It is worth noting that the indispensable cropping in U-Net is unnecessary in our network. The parameters and output size of each step are presented in Table I.(rewrite = Resunet paper)


%In this work, we utilize a 4-level architecture of Resunet++ for extraction of the polyp features. At the last part of the network, we recover the representation to pixel wise categorization. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Experiments}



\subsection{Dataset}
The Kvasir polyp dataset consist of 1000 images with  resolution from 720$\times$576 to 1920$\times$1072 pixels. The CVC-ColonDB consist of 356 low-resolution images of size 500$\times$574. The CVC-ClinicDB database contains 612 images of size 384$\times$288 resolution. The CVC-12K dataset consists of images with the image size 384$\times$288 resolution. 

The labelbox~\cite{Labelbox} toolbox is used for marking the polyp region out of the entire image frame. We have released the corresponding mask for the Kvasir dataset. Now, multimedia researchers can use both images and ground truth information for comparing methods and experimental results. A polyp example from kvasir dataset and the generated corresponding mask is shown in Figure~\ref{fig:polyp_with_mask}.


We have evaluated our proposed architecture using the Kvasir-SEG dataset, CVC-ColonDB (CVC-356)~\cite{bernal2017comparative}, CVC-ClinicDB (CVC-612)~\cite{bernal2015wm}, CVC-912, and CVC-12k~\cite{bernal2017comparative} dataset. The Kvasir polyp dataset consist of 1000 images with  resolution from 720$\times$576 to 1920$\times$1072 pixels. The CVC-ColonDB consist of 356 low-resolution images of size 500$\times$574. The CVC-ClinicDB database contains 612 images of size 384$\times$288 resolution. The CVC-12K dataset consists of images with the image size 384$\times$288 resolution. 


\subsection{Data preprocessing}
%The tensorflow version used is 1.8.0. 


%for reference see ResUNet paper


%we train and validate the models with one dataset and test on theand test the model on completely new dataset to see how well the proposed architecture performs on the completely new dataset.  

% Again, we use unseen dataset for testing the performance of the model. Speed is also an important parameter for clinical acceptability. Hence, we measured polyp detection rate. 







%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Discussion}
We would like to acknowledge that the performance curves
reported for different models and applications may not be the
best that we could achieve for each experiment. This suboptimal performance is related to the choice of the hyperparameters of CNNs that can influence the speed of convergence and final accuracy of a model.

Although we attempted to find the working values of these parameters, finding the
optimal values was not feasible given the large number of CNNs studied in our paper and that training each CNN was a time-consuming process even on the high-end GPUs.  Nevertheless, this issue may not change our overall conclusions as the majority of the CNNs used in our comparisons are pre-trained models that may be less affected by the choice of hyper-parameters than the CNNs trained from scratch.


%%%%%%%##########Discussion%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



Different methods have been proposed to tackle the problem of creating CNNs designed to be an efficient architecture for pixel-wise semantic segmentation.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Data augmentation can be useful, as shown in this study, but the trade-off between computational burden and classification needs to be made. Potentially, larger and deeper convolutional neural networks could be applied to further improve classification performance [59], [60]. However, the curse-of-dimensionality problem makes it difficult to assess the amount of necessary data that is needed to effectively train these very deep networks.
Extensions of ConvNets to 3D have been proposed, but computational cost and memory consumption can be still too high to efficiently implement them on current computer graphics hardware units [23].

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Description of the Result Comparison}
%Discuss which type of image you are missing
%One of the challenges in the polyp segmentation task is the dataset. Some of the polyp frame are underexposed, overexposed, the images are taken so close, blurring, overlay information, and overexposed regions. The dataset used for training and testing comes from different sources and are captured using different devices. These variability resolution may affect the performance of our model. 
%However, the huge difference in the model performance shows that it is hard to obtain generalizable model especially when we do experiment with images captured using different instruments. 
%Using more image augmentation would not increase the training accuracy but only increase the training complexities. 
%We have averaged the results per image to obtain the overall automatic segmentation performance compared with the ground truth images. (rewrite)

%%%%%%%%%%%%%%%%%%%%%%%%%experiment%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
According to our exploratory experiments,the learning rate and scheduling rate heavily influenced the convergence of CNNs. A learning rate of 0.001 however ensured proper convergence for all 4 applications. A smaller learning rate slowed down convergence and a larger learning rate often caused convergence failures.



We then averaged the probabilistic outputs of the test patches at the candidate level and performed an FROC analysis for performance evaluation.




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{some more discussions}

A major strength of CADe systems is that they are not susceptible to inherent
inter- and intra-observer variability, and can therefore improve ADRs regardless of
the endoscopist’s skill. 

data-privacy considerations


%In images where the foreground object tend to vary a bit therein, U-Net, was unable to segment the foreground as a continuous region. It rather predicted a set of scattered regions (Fig. 9a), confusing the foreground as background and thus caused the loss of some valuable information. On the other hand, for images where the background is not uniform, the U-Net model seems to make some false predictions (Fig. 9b). The more rough the background becomes, the more false predictions are made (Fig. 9c). Furthermore, in some dreadfully adverse situations, where due to irregularity the difference between background and foreground are too subtle, the U-Net model failed to make any predictions at all (Fig. 9d). Although in such challenging cases the segmentation of MultiResUNet is not perfect, it performs far superior than the classical U-Net model as shown in Fig. 9.

%The ideal automatic polyp segmentation and detection software should have (1) high overall performance (2) Uniform performance on a specific image and (3) low latency.  




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Conclusion}
In conclusion, automatic algorithms can assist endoscopists in identifying polyps that are adenomatous but have been incorrectly judged as hyperplasia
and, therefore, enable timely resection of these polyps at
an early stage before they develop into invasive cancer.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Reference and citation}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

https://arxiv.org/pdf/1705.03820.pdf
Data augmentation from here

there are significant limitations due to the limited background variability

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Some nice terms to use in paper
we investigate
Panel of experts
explicitly



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Interesting paper}
https://arxiv.org/pdf/1806.01907.pdf


Remaining figures
\section{no of filters graph}

% \begin{table}[]
% \label{convolutional_kernel}
% \def\arraystretch{1.1}
%  \setlength\tabcolsep{8pt}
% %\centering
% \caption{Number of Convolutional filters used in U-Net, Resunet and \resunetplusplus}
% \begin{tabular}{|l|r|r|r|r|r|}
% \hline
% \bf Encoder/decoder & X0,0   & X1,0    & X2,0   & X3,0    & X4,0 \\ \hline
% %\bf Encoder/decoder & X0,0/X0,4   & X1,0/X1,3    & X2,0/X2,2    & X3,0/X3,1    & X4,0/X4,0\\ \hline
% U-Net   & 32    & 64    & 128   & 256  & 512\\ \hline
% Resunet  & 64    & 128   & 256   & 512 & 1024 \\ \hline
% \resunetplusplus & 16   & 32   & 64  & 128   & 256 \\ \hline
% \end{tabular}
% \end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

